PDP: Physics-Based Character Animation via Diffusion Policy

Generating diverse and realistic human motion that can physically interact with an environment remains a challenging research area in character animation. Meanwhile, diffusion-based methods, as proposed by the robotics community, have demonstrated the ability to capture highly diverse and multi-modal skills. However, naively training a diffusion policy often results in unstable motions for high-frequency, under-actuated control tasks like bipedal locomotion due to rapidly accumulating compounding errors, pushing the agent away from optimal training trajectories. The key idea lies in using RL policies not just for providing optimal trajectories but for providing corrective actions in sub-optimal states, giving the policy a chance to correct for errors caused by environmental stimulus, model errors, or numerical errors in simulation. Our method, Physics-Based Character Animation via Diffusion Policy (PDP), combines reinforcement learning (RL) and behavior cloning (BC) to create a robust diffusion policy for physics-based character animation. We demonstrate PDP on perturbation recovery, universal motion tracking, and physics-based text-to-motion synthesis.

==> experiments_old.tex <==
% \subsection{Problem Statement}
% \zhaoming{It may be better to restructure like this:
% 1. Method Section: General description of the problem: Given expert trajectories, $o_t, a_t$, do diffusion + DASS + model architecture.
% 2. Experiment Section: Describe Task here + what is already here
% }

% \subsubsection{Tasks} We apply our method to two popular motion generation tasks. The first task is text-to-motion, which is the task of generating motion given a text prompt. The input is a text prompt (a short description or command) in natural language and the output is the resulting motion. Because our focus is physics-based character animation, we also expect the output motion to adhere to physics. The second task is motion tracking, where the model is provided a reference motion state at each timestep that it attempts to match.

% \subsubsection{Observation Space} We use different observations for text-to-motion than motion tracking. For both tasks, we use the humanoid model from \cite{luo2023_PHC}, which follows the SMPL kinematic structure with $J = 24$ links, of which 23 are actuated. The observation space for the text-to-motion task takes the form $o_t^{T2M} = (\bm{x}^p, \bm{x}^r, \dot{\bm{x}}^p, \dot{\bm{x}}^r)$, where $\bm{x}^p \in \mathbb{R}^{3J}$ is the local position of each skeleton link, $\bm{x}^r \in \mathbb{R}^{6J}$ is the 6D rotation \cite{6D_rot}, $\dot{\bm{x}}^p \in \mathbb{R}^{3J}$ is the linear velocity in the character frame, and $\dot{\bm{x}}^r \in \mathbb{R}^{3J}$ is the angular velocity.

% The observation space for the motion tracking task contains similar elements as that of the text-to-motion task, except it contains the difference of each element with the corresponding element in the reference motion. Then the resulting observation is concatenated with the position and rotation of reference motion observation itself. Concretely, the observation takes the form $o_t^{MT} = (\Delta\bm{x}^p, \Delta\bm{x}^r, \Delta\dot{\bm{x}}^p, \Delta\dot{\bm{x}}^r, \bm{x}^{p}_{ref}, \bm{x}^r_{ref})$, where $\Delta\bm{x}^p = \bm{x}^{p}_{ref} - \bm{x}^p$ and the other $\Delta$ terms are similarly defined.

% \subsubsection{Action Space} For both tasks, we use proportional derivative (PD) targets of the 23 actuated joints in our humanoid model are our action $a_t$, resulting in a 69-dimensional action space.

% Talk about how the noisy trajectories can be viewed as multiple trajectories each with a single step. 
% \subsubsection{Model Architecture} In our approach, we adapt the transformer architecture from the Diffusion Policy model, tailoring it to align with the data collection process of DASS. Specifically, rollouts from DASS can be conceptualized as a series of one step trajectories or episodes. This unique structure emerges because at every timestep, a noisy action is employed to advance the simulator. 

% From the standpoint of predicting the current corrective action, its dependency on preceding corrective actions within the rollout is relatively tenuous. This is because the previous corrective actions in the sequence are far more dependent on noise then 

% For example it does not make sense for the model to predict a sequence of corrective actions because those actions themselves were dependent on being in a sub-optimal state. In this same idea, preceding the current action based on the sequence of previous corrective actions appear as noise. To optimize this model, we removed the initial multi-headed attention mechanism from the decoder layer. 

% One reason to predict the horizon is that it can help contextualize the current action, and reduce its error, which reduces the chance of visiting a sup-optimal or out of distribution state. However, given the sampling method, the predicted action does not need to be perfect, because we give corrective feedback. 

\section{Experiments}

% \zhaoming{where are the specialized policies come from? give details of how it is obtained, and how the dataset is collected.}

\subsection{Tasks}\label{sec:tasks}
We apply our method to two motion generation tasks. For both tasks, explained below, we use the humanoid model from \cite{luo2023_PHC}, which follows the SMPL kinematic structure with $J = 24$ links, of which 23 are actuated. We will first define some notation to make it easier to explain the observations and actions for each task. All quantities are in character frame unless otherwise stated. $\bm{x}^p \in \mathbb{R}^{3J}$ is the center of mass position of each joint body, $\bm{x}^r \in \mathbb{R}^{6J}$ is the 6D rotation \cite{6D_rot}, $\dot{\bm{x}}^p \in \mathbb{R}^{3J}$ is the linear velocity, and $\dot{\bm{x}}^r \in \mathbb{R}^{3J}$ is the angular velocity.

\paragraph{Motion Tracking} In the motion tracking task, the goal is to match a known reference motion at each timestep. At each timestep, the policy receives information about the reference motion state. In our setup, the policy receives $\bm{x}^{p}_{ref}$ and $\bm{x}^r_{ref}$, which are the center of mass position of each body of the reference motion and the 6D rotation of the reference motions, respectively. The full motion tracking observation $\bm{o}_t^{MT}$ can then be defined as a tuple $(\Delta\bm{x}^p, \Delta\bm{x}^r, \Delta\dot{\bm{x}}^p, \Delta\dot{\bm{x}}^r, \bm{x}^{p}_{ref}, \bm{x}^r_{ref})$, where $\Delta\bm{x}^p = \bm{x}^{p}_{ref} - \bm{x}^p$ and the other $\Delta$ terms are similarly defined. We use proportional derivative (PD) targets of the 23 actuated joints in our humanoid model as our action $\bm{a}_t$, resulting in a 69-dimensional action space.

\paragraph{Text to Motion} In the text-to-motion task, the goal is to generate motion conditioned on a natural language text prompt. The policy receives the natural language text prompt as input, which is encoded using CLIP before being combined with the observation. The observation takes the form $\bm{o}_t^{T2M} = (\bm{x}^p, \bm{x}^r, \dot{\bm{x}}^p, \dot{\bm{x}}^r)$. The action space is the same as in the motion tracking task.

\subsection{Training Diffusion Policies}
We train PDP using a denoising process with $K=100$ steps and a cosine noise schedule. For experiments using KIT, we train on 4 \textit{NVIDIA A100} GPUs for approximately 12 hours. For experiments using AMASS, we train with the same hardware for approximately 36 hours.

The training dataset consists of state-action trajectories generated by RL policies. Since our method is agnostic to the RL policies themselves, we utilize pre-trained motion tracking controller PHC \cite{luo2023_PHC} to track most of the motions and train individual policies for challenging motions where PHC fails \cite{2018-TOG-deepMimic}. With PHC and a few specialized small policies, our training set covers most motions in AMASS \cite{amass2019} and KIT \cite{plappert2016kit}, excluding motions that interact with chairs, lean on tables, and motions that are similarly infeasible in our physics simulator, following the same practice in PHC.

\paragraph{Motion Tracking}
We shuffle motions in AMASS to produce training, validation, and test sets, with splits $80\%$ $10\%$, and $10\%$, respectively. PHC can successfully track most trajectories in its training set, but still requires a few specialized RL policies additionally trained by us to complete the rollout generation for the entire training set. For these motions we exclude them from the initial training and put them into a new dataset where we then demonstrate the models ability to adapt to challenging and new tasks through fine-tuning. 

\paragraph{Text to Motion}
We use KIT dataset and the text annotations from HumanML3D \cite{guo2022Humanml3d}, following the common practice of existing text-to-motion methods, such as MDM \cite{tevet2023human}. The task vector is generated through the CLIP embedding of the text annotation and motion tracking policies are used to generate the observation-action trajectories for each text.

%We evaluate on two datasets: AMASS \cite{amass2019} and KIT \cite{plappert2016kit}. AMASS is a large dataset of human motion with over 11000 motions and more than 40 hours of motion data. KIT is a subset of AMASS that contains 3911 motions, and is included for a more direct comparison to works like MDM \cite{tevet2023human}. For both datasets, we follow the practice in \cite{luo2023_PHC} of removing motions that interact with chairs, lean on tables, and motions that are similarly infeasible in our physics simulator, resulting in 11626 motions for AMASS and 3628 motions for KIT. For the text annotations, we used HumanML3D \cite{guo2022Humanml3d}, a large dataset containing the same motions and KIT and AMASS along with multiple text annotations per motion.

\subsection{Baselines}
For motion tracking, we compare against the SOTA motion tracking method PHC \cite{luo2023_PHC}. We also ablate the amount of data PDP sees during training to show the strong generalization capabilities offered by diffusion models. We experiment with 100\% of the training data (PDP-100), 50\% (PDP-50) and 25\% (PDP-25). 

For text-to-motion, since most existing text-to-motion methods are kinematics-based, we train a vanilla Diffusion Policy using the same training data and the same text embedding architecture as our method. The main difference of this baseline from PDP is that it uses clean-state-action trajectories as training data, and it uses self attention over actions. Specifically, we compare the robustness of generated motions through text. 

\subsection{Evaluation Metrics} 
 We evaluate the success rate of motion tracking, where success is defined as in PHC. Namely, the episode is considered a failure if at any point during evaluation the joints are more than $0.5m$ from the reference motion. We also adopt the same metrics used by \cite{luo2023_PHC}. Namely, mean per-joint position error $E_{\text{mpjpe}}$ and global mean per-joint position error $E_{\text{g-mpjpe}}$, which measure the ability of the model to accurately match the reference motion in the local and global frames. We also measure the error in velocity $E_{\text{vel}}$ and acceleration $E_{\text{acc}}$ between the simulated character and the motion capture data. 


% We adopt the metrics suggested by \cite{Guo_2022_CVPR} for text-to-motion: \textit{R-precision} and \textit{Multimodal-Dist} measure how relevant the resulting motion is to the input prompt, \textit{Fréchet Inception Distance (FID)} measures the distance between the ground truth motion distribution and the generated motion distribution, \textit{Diversity} measures the variance of all motions across all text prompts, and \textit{MultiModality} measures the variance of the motions generated given a particular text command.

==> extra/method_old.tex <==
\subsection{Background}

\subsubsection{Diffusion Policies}
% Diffusion models effectively capture complex multi-modal data distributions and offer more stable training compared to other generative model classes. These properties make diffusion models a desirable choice for text-conditioned motion generation, where many different motions may be a valid match for any particular text description. 

Denoising Diffusion Probabilistic Models (DDPMs) \cite{ho2020ddpm} are a type of diffusion model where sampling is achieved through a denoising process known as Stochastic Langevin Dynamics \cite{welling2011bayesian} starting from pure random noise. The denoising process is learned by a noise-prediction network $\epsilon_{\theta}(x^k, k)$, where $x^k$ is the noisy data at diffusion step $k$ and $\theta$ is the set of learned model parameters. The denoising process is given by

\begin{equation}
    x^{k-1} = \alpha (x^k - \gamma \epsilon_{\theta}(x^k, k) + \mathcal{N}(0, \sigma \bm{I})),
\end{equation}

\noindent
where $\alpha, \gamma$ and $\sigma$ are hyper-parameters called the noise schedule, and may or may not depend on $k$. The noise-prediction model is learned in a self-supervised manner using the mean squared error objective 

\begin{equation}
    \mathcal{L} = MSE(\epsilon^k, \epsilon_{\theta}(x^0 + \epsilon^k, k)).
\end{equation}

Diffusion policies \cite{chi2023diffusionpolicy} introduced DDPMs to the domain of robotic control. In particular, the denoising process operates on noisy action trajectories $\bm{a}_{1:T}$, where $a_t$ is the action taken by a controller at timestep $t$ and $T$ is the control horizon. At each diffusion step, the noise-prediction model denoises an entire noisy trajectory $\bm{a}_{1:T}^k$.


% Given a data distribution $p(\bm{X})$, two stochastic processes are modeled, a forward and a reverse process. In the forward process, a sample $x \sim p(\bm{X})$ and an integer $k \in [1, K]$ are sampled, then $k$ steps of Gaussian noise is applied to $x$, inducing $K$ conditional Gaussian distributions of the form $p_{k}(x^k \mid x)$ over noisy data.

% \begin{equation}
%     p_{k}(x^k \mid x) = p(x)\prod_{i=1}^{k} p_{i}(x^i \mid x^{i-1})
% \end{equation}

% \noindent
% In the reverse process, the learned noise prediction model $\epsilon_{\theta}(x^k, k)$ predicts the noise applied to $x^{k-1}$ to produce $x^k$ in iteration $k$ of the forward process. During inference, a sample is produced by starting from pure noise, which approximates $x^K$, then the model runs $K$ iterations of the reverse process to produce clean data $x^0$. In particular, the reverse process is computed using Stochastic Langevin Dynamics, and following the equation

% \begin{equation}
%     x^{k-1} = \alpha (x^k - \gamma \epsilon_{\theta}(x^k, k) + \mathcal{N}(0, \sigma \bm{I})),
% \end{equation}

% \noindent
% where $\alpha, \gamma$ and $\sigma$ are hyper-parameters called the noise schedule, and may or may not depend on $k$. The noise prediction network $\epsilon_{\theta}$ is learned in a self-supervised manner using the mean squared error objective 

% \begin{equation}
%     \mathcal{L} = MSE(\epsilon^k, \epsilon_{\theta}(x^0 + \epsilon^k, k)).
% \end{equation}

% Diffusion policies \cite{chi2023diffusionpolicy} introduce DDPMs to the domain of robotic control. In particular, the data distribution $p(\bm{X})$ now becomes a distribution over action trajectories $p(\bm{a}_{1:T})$, where $a_t$ is the action taken by a controller at timestep $t$, $T$ is the control horizon, and diffusion iteration $k$ is applied to the entire trajectory to produce $\bm{a}_{1:T}^{k}$. 

\subsubsection{Robust Behavioral Cloning}
% Talk about Behvaioural Cloning
Behavioral Cloning (BC) has been applied to real world robotic tasks such as manipulation \cite{florence2019selfsupervised}, driving  \cite{pomerleau1988alvinn}, and bipedal locomotion \cite{xie2020learning}. However, a significant challenge it faces is the problem of compounding errors. This issue emerges because the deterministic expert policy, used to collect training data for the student, only covers the trajectory's optimal states and actions. As a result, the studeent policy lacks exposure to slightly sub-optimal states, which can occur due to model errors or noise during rollout. Diffusion Policy, also trained via behavioural cloning, is not exempt from this challenge. We observe that naively training the diffusion policy struggles with robustness in character control. 

One strategy to mitigate this problem involves augmenting the training dataset with corrective actions derived from visiting sub-optimal states. DAGGER, for instance, uses the BC policy to explore sub-optimal states, then samples the expert policy for corrections which is added back to the dataset and re-trained \cite{ross2011reduction}. DART extends the exploration of the state space by rolling out the expert policy with a learned noise level. Simplifying this concept further, DASS eliminates the need for determining optimal noise levels, and has shown promising results in robust bipedal walking with the Cassie robot. \cite{pmlr-v100-xie20a}. In our work, we leverage the DASS methodology to compile a dataset enriched with corrective actions.

==> results.tex <==
\section{Results}

% Table
\begin{table}[t]
\centering
\begin{minipage}{\columnwidth}
\begin{center}
%\scriptsize % Uncomment this to reduce text size
\resizebox{\textwidth}{!}{
\begin{tabular}{c c c c c c}
  \toprule
    Method & Success (\%) \uparrow & E_{\text{g-mpjpe}} \downarrow & E_{\text{mpjpe}} \downarrow & E_{\text{vel}} \downarrow & E_{\text{acc}} \downarrow \\ \midrule 
    PHC (Upper Bound) & 99.6 & 36.8 & 27.0 & 2.9 & 4.3 \\ \midrule 
    PDP-100 & 90.6 & 36.8 & 26.4 & 3.8 & 4.6 \\
    PDP-50 & 89.9 & 37.2 & 26.5 & 3.8 & 4.6 \\
    PDP-25 & 89.0 & 37.4 & 26.4 & 3.9 & 4.7 \\
  \bottomrule
\end{tabular}
}
\end{center}
\caption{Motion Tracking results on AMASS* Test Dataset}
\label{tab:amass-mt}
\end{minipage}
\end{table}


% % Table
% \begin{table}[t]
% \centering
% \begin{minipage}{\columnwidth}
% \begin{center}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c c c c c c}
%   \toprule
%     Method & Succ (\%) & FID & R-Precision (top-3) & Multimodal Dist & Diversity \midrule 
%     Diffusion Policy &  \\ \midrule
%     %PDP-Upsampled (Ours) & {\color{green}Running} \\
%     PDP (Ours) & 9.86^{\pm 0.15} & 0.36^{\pm 0.01} & 5.75^{\pm 0.03} & 6.56^{\pm 0.06} \\ \bottomrule
% \end{tabular}
% }
% \end{center}
% \caption{Text-to-motion results on the KIT* dataset.}
% \label{tab:kit-t2m}
% \end{minipage}
% \end{table}%






% \begin{table}[t]
% \centering
% \begin{minipage}{\columnwidth}
% \begin{center}
% \scriptsize
% \begin{tabular}{c c c c c c c}
%   \toprule
%     Method & Succ (\%) & FID & R-Precision & Multimodal Dist & Diversity & MM \\ \midrule 
%     InsActor & & \\ 
%     Diffusion Policy & {\color{blue} Ready to Run}  \\ \midrule
%     PDP-NRTM (Ours) & {\color{blue} Ready to Run} \\
%     PDP (Ours) & {\color{green}Running} \\ \bottomrule
% \end{tabular}
% \end{center}
% \caption{Text-to-motion results on the cleaned AMASS dataset.}
% \label{tab:amass-t2m}
% \end{minipage}
% \end{table}%



% Table
\begin{table}[t]
\centering
\label{tab:kit-mt}
\begin{minipage}{\columnwidth}
\begin{center}
%\scriptsize % Uncomment this to reduce text size
\begin{tabular}{c c c c c c}
  \toprule
  Method & Success (\%) \\ \midrule
   Vanilla DP w/o DASS & 52.0 \\ \midrule
   PHC w/o DASS & 8.0 \\ 
    PHC + DASS & 99.0\\ 
  \bottomrule
\end{tabular}
\end{center}
\caption{Ablation on Sampling Procedures}
\end{minipage}
\end{table}%

% \begin{figure*}[h]
% \includegraphics[width=0.8\textwidth]{example-image-c}
% \caption{A figure to depict motion tracking and text-to-motion results.}
% \label{fig:mt_t2m_results}
% \end{figure*}

% \begin{figure*}[ht]
%     \centering
%     \begin{subfigure}[b]{0.45\textwidth} % Subfigure a
%         \centering
%         \includegraphics[width=\textwidth]{example-image-c}
%         \caption{A figure to depict motion tracking results.}
%         \label{fig:mt_results}
%     \end{subfigure}
%     \hfill % Optional: adds horizontal space between subfigures
%     \begin{subfigure}[b]{0.45\textwidth} % Subfigure b
%         \centering
%         \includegraphics[width=\textwidth]{extra/mouse.pdf}
%         \caption{A figure to depict text-to-motion results.}
%         \label{fig:t2m_results}
%     \end{subfigure}
%     \caption{Caption for the whole figure}
%     \label{fig:test}
% \end{figure*}



\subsection{Comparison with Baselines}

We demonstrate that PDP is capable of tracking a significant portion of AMASS* dataset\footnote{* indicates removing sequences containing human-object interaction for both the AMASS and KIT datasets and using motions that PHC succeeds on.} reliably, Table \ref{tab:amass-mt}. Because we use PHC to collect our dataset for imitation learning, PHC represents an upper bound for the AMASS* test dataset. In Section \ref{sec:hardmotions}, we demonstrate that our model is able to adapt to new tasks quickly, as explained in Section \ref{sec:experiments}.

Our method achieves $90.6\%$ success rate on the AMASS* test dataset. Furthermore, the table shows that PDP has strong generalization capabilities: PDP achieves nearly the same test set performance, $89.9\%$ using $50\%$ of the AMASS* training data and $89.0\%$ success rate using only 25\% of the training data. PDP also achieves comparable MPJPE and global MPJPE as PHC, indicating a close approximation to the target motion.
% Figure \ref{fig:mt_results} depicts the results of our motion tracking method, where it is clear that PDP is capable of tracking the complex and diverse distribution of motions present in AMASS*. 

% Table \ref{tab:kit-t2m} shows our results on the text-to-motion task on the KIT* dataset. We compare our method against vanilla diffusion policy. Our method achieves \michael{TODO} FID. Figure \ref{fig:t2m_results} shows our method generating a diverse range of text-conditioned motions, highlighting the ability of diffusion models to capture multimodal distributions.

% \begin{itemize}
%     \item Text2motion generation can be validated using (FID, R-precision, Multi-modal distance,  diversity) Compare to Instactor and PADL. Motion tracking, RSME on joint positions compared to original PHC. 
%     \item Compare our noisy sampling strategy to long horizon learning.  
%     \item Find a set of motions where PHC fails, train a few local expert policies and finetune. compared to fine-tuning PHC.  

% \end{itemize}


\subsection{Ablations}
% \zhaoming{what are some key components that make the system work? We can put them here.}
In this section, we demonstrate the necessity of incorporating state exploration for the policy to learn effectively. We compare the performance of our architecture using DASS against its performance without DASS, as well as against the vanilla diffusion policy which predicts future actions. To assess their effectiveness, we perform text-conditioned rollouts, where the success rate is determined by whether the character remains active (not terminated or fallen) within an 8-second window.

Our results indicate a striking difference in performance: using DASS yields a 99\% success rate, a significant improvement over the 8\% success rate when our architecture operates without DASS. In comparison, the vanilla diffusion policy achieves a 52\% success rate. These findings suggest that while predicting future actions may contribute to robustness, the integration of DASS into our architecture is substantially more effective in ensuring successful outcomes.


% \begin{table}[h]
% \centering
% \begin{minipage}{\columnwidth}
% \begin{center}
% %\scriptsize % Uncomment this to reduce text size
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{c c c c c c}
%   \toprule
%     Method & Success (\%) \uparrow & E_{\text{g-mpjpe}} \downarrow & E_{\text{mpjpe}} \downarrow & E_{\text{vel}} \downarrow & E_{\text{acc}} \downarrow \\ \midrule 
%     PHC & - & \\ 
%     PDP-100 & \\
%     PDP-Hard & \\ \bottomrule
% \end{tabular}
% }
% \end{center}
% \caption{Motion Tracking results on AMASS-Hard}
% \label{tab:pdp-hard}
% \end{minipage}
% \end{table}%


\subsection{Adapting to New Motions}\label{sec:hardmotions}
% \michael{Section describing how we trained motion tracking policies on the 131 AMASS motions that PHC fails to track and easily distilled them into PDP. Then we can claim 100\% success on AMASS.}
In order to showcase the ability of PDP to quickly adapt a new task, we train a separate policy and fine-tune the pretrained model. We then re-evaluate it on the test set to check for any catastrophic forgetting. For this task, we fine-tuned on a handstand motion where PHC failed to track. After training a specialized RL policy for this task, we collect noisy rollouts following DASS procedure. We then fine-tune on this small dataset which only takes 1500 epochs to train, or about 5-8 minutes on a single GPU. 

% train a separate collection of expert policies on this dataset of 131 motions, which we call "AMASS-Hard" using AMP \cite{peng2021amp}. We then distill the resulting policies into PDP using the AMASS* train dataset that PDP was trained on combined with the dataset generated by these separate experts. By definition, PHC achievs a 0\% success rate on AMASS-Hard. Table \ref{tab:pdp-hard} shows that PDP is able to easily distill the expert policies and outperform PHC, achieving as success rate of \michael{TODO} on AMASS-Hard. 

% We demosntrate that the diffusion policy has strong generalization capabilities \ref{tab:amass-mt}. Interestingly, despite being more difficult than the data distribution these policies were trained on, they are still able to generalize zero-shot and achieve impressive success rates of \michael{TODO}, \michael{TODO}, and \michael{TODO}, respectively.

% \begin{figure}[h]
% \includegraphics[width=0.45\textwidth]{figures/plot.png}
% \caption{A figure to show results on AMASS-Hard \michael{This is a placeholder figure. Not real data.}}
% \label{fig:pdp_hard}
% \end{figure}





